Neuromorphic Imaging with Super-Resolution

Neuromorphic imaging is an emerging technique that imitates the human retina to sense variations in dynamic scenes. It responds to pixel-level brightness changes by asynchronous streaming events and boasts microsecond temporal precision over a high dynamic range, yielding blur-free recordings under extreme illumination. Nevertheless, this modality falls short in spatial resolution and leads to a low level of visual richness and clarity. Pursuing hardware upgrades is expensive and might cause compromised performance due to more burdens on computational requirements. Another option is to harness offline, plug-in-play super-resolution solutions. However, existing ones, which demand substantial sample volumes for lengthy training on massive computing resources, are largely restricted by real data availability owing to the current imperfect high-resolution devices, as well as the randomness and variability of motion. To tackle these challenges, we introduce the first self-supervised neuromorphic super-resolution prototype. It can be self-adaptive to per input source from any low-resolution camera to estimate an optimal, high-resolution counterpart of any scale, without the need of side knowledge and prior training. Evaluated on downstream tasks, such a simple yet effective method can obtain competitive results against the state-of-the-arts, significantly promoting flexibility but not sacrificing accuracy. It also delivers enhancements for inferior natural images and optical micrographs acquired under non-ideal imaging conditions, breaking through the limitations that are challenging to overcome with frame-based techniques. In the current landscape where the use of high-resolution cameras for event-based sensing remains an open debate, our solution is a cost-efficient and practical alternative, paving the way for more intelligent imaging systems.

==> src/table_intro_comp.tex <==
\begin{table}[t]
\caption{Evaluations of existing neuromorphic SR methods}
\label{table:intro_comp}
\centering
\begin{threeparttable}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}} lccccc}
    \toprule
    \textbf{Method} & \#1 & \#2 & \#3 & \#4 & \#5\\ \midrule
    Li~\etal~\cite{li2019neurocomputing} & \xmark & \cmark & \cmark & \xmark & \xmark\\
    Wang~\etal~\cite{wang2020cvpr} & \xmark & \xmark & \cmark & \xmark & \cmark\\
    Duan~\etal~\cite{duan2021cvpr} & \cmark & \xmark & \xmark & \xmark & \xmark\\
    Li~\etal~\cite{li2021iccv} & \cmark & \xmark & \xmark & \cmark & \xmark\\ 
    Weng~\etal~\cite{weng2022eccv} & \cmark & \xmark & \xmark & \xmark & \cmark\\ \midrule
    Ours & \cmark &  \cmark&  \cmark & \cmark & \cmark\\
    \bottomrule
\end{tabular*}
\begin{tablenotes}
    \item[1] Learning-based method?
    \item[2] Free of auxiliary data?
    \item[3] Free of prior training?
    \item[4] Spatiotemporal SR performed?
    \item[5] Large-scale (\eg, $8 \times$, $16 \times$) SR achieved?
\end{tablenotes}
\end{threeparttable}

\end{table}
